Deciphering Cell Systems: Machine Learning Perspectives And Approaches For The Analysis Of Single-Cell Data

This dissertation explores the application of machine learning in molecular biology, focusing on gene expression regulation and cellular behavior at the single-cell level. Using modern neural networks, the research addresses key challenges in cell-cell communication, gene function inference, and protein expression analysis, with a special focus on single-cell RNA sequencing (scRNA-seq) data. Advanced computational methodologies integrating systems biology and neural network techniques were developed to handle the complexity and high-dimensionality of single-cell data, leading to a deeper understanding of genotype-phenotype relationships. This work proposes novel solutions to optimization problems in manifold learning, explores generative models for gene regulatory networks, and simulates gene knockout at single-cell resolution. Furthermore, the research enhances the interpretability of black-box neural models for multimodal data. Key contributions to cellular biology include the analysis of cell-cell interactions and their role in shaping cellular behavior, gene function prediction through knockout simulations, and the investigation of how gene expression patterns translate into protein expression. These findings have implications for understanding disease mechanisms and therapeutic development. Overall, this dissertation advances computational biology by providing new tools and insights into single-cell analysis, offering a valuable resource for future studies on cellular behavior and potential treatments for various diseases.

==> data/nomenclature.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
% 
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           NOMENCLATURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{NOMENCLATURE}
\addcontentsline{toc}{chapter}{NOMENCLATURE}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.

%A note about aligning: These entries will align
%themselves according to the ampersand (&).
%No extra spaces are needed, as seen in some of
%the entries below.

%Example of the longtable environment.
\hspace*{-1.25in}
\vspace{12pt}
\begin{spacing}{1.0}
	\begin{longtable}[htbp]{@{}p{0.35\textwidth} p{0.62\textwidth}@{}}
	   % \begin{tabular}{@{}p{0.33\textwidth} p{0.62\textwidth}@{}}
		OGAPS	&	Office of Graduate and Professional Studies at Texas A\&M University\\	[2ex]
		B/CS		&	Bryan and College Station\\	[2ex] %[2ex] provides double space between each row
		TAMU			&	Texas A\&M University\\	[2ex]
		SDCC & San Diego Comic-Con\\ [2ex]
		EVIL & Every Villain is Lemons\\ [2ex]
		EPCC & Educator Preparation and Certification Center at Texas A\&M University - San Antonio\\ [2ex]
		FFT & Fast Fourier Transform\\ [2ex]
		ARIMA & Autoregressive Integrated Moving Average\\ [2ex]
		SSD & Solid State Drive\\ [2ex]
		HDD & Hard Disk Drive\\ [2ex]
		O\&M & Eller Oceanography and Meteorology Building\\ [2ex]
		DOS & Disk Operating System\\ [2ex]
		HDMI & High Definition Multimedia Interface\\ [2ex]
		$L^1$ & Space of absolutely Lebesgue integrable functions; i.e., $\int |f| < \infty$\\ [2ex]
		$L^2$ & Space of square-Lebesgue-integrable functions, i.e., $\int |f|^2 < \infty$\\ [2ex]
		$PC(S)$ & Space of piecewise-continuous functions on $S$\\ [2ex]
		GNU & GNU is Not Unix\\ [2ex]
		GUI & Graphical User Interface\\ [2ex]
		PID & Principal Integral Domain\\ [2ex]
		MIP & Mixed Integer Program\\ [2ex]
		LP & Linear Program\\ [2ex]
		%XXXXXXXX		&	This is an optional page. Random word to test how long the sentence can be? This is just for test purpose. The current setting aims to align left/right margin same as all other pages.\\	[2ex]
	   % \end{tabular}%
	\end{longtable}
\end{spacing}

\pagebreak{}
